Self-Exploring Language Models: Active Preference Elicitation for Online Alignment

Preference optimization, particularly through Reinforcement Learning from Human Feedback (RLHF), has achieved significant success in aligning Large Language Models (LLMs) to adhere to human intentions. Unlike offline alignment with a fixed dataset, online feedback collection from humans or AI on model generations typically leads to more capable reward models and better-aligned LLMs through an iterative process. However, achieving a globally accurate reward model requires systematic exploration to generate diverse responses that span the vast space of natural language. Random sampling from standard reward-maximizing LLMs alone is insufficient to fulfill this requirement. To address this issue, we propose a bilevel objective optimistically biased towards potentially high-reward responses to actively explore out-of-distribution regions. By solving the inner-level problem with the reparameterized reward function, the resulting algorithm, named Self-Exploring Language Models (SELM), eliminates the need for a separate RM and iteratively updates the LLM with a straightforward objective. Compared to Direct Preference Optimization (DPO), the SELM objective reduces indiscriminate favor of unseen extrapolations and enhances exploration efficiency. Our experimental results demonstrate that when fine-tuned on Zephyr-7B-SFT and Llama-3-8B-Instruct models, SELM significantly boosts the performance on instruction-following benchmarks such as MT-Bench and AlpacaEval 2.0, as well as various standard academic benchmarks in different settings. Our code and models are available at https://github.com/shenao-zhang/SELM.

==> method.tex <==
\section{Method}
With the above motivation, we propose to augment the data by conditioning the preference pairs on the reward values. Specifically, we define the goal-conditioned reward $r_g(x, y) = \1\bigl(g=r(x, y)\bigr)$ as a function of the reward value $r$ given by the judge model. The objective of the reward-conditioned policy $\pi(y\mid x ; g)$ is to minimize the absolute difference between the goal reward $g$ and the response quality $r(x, y)$, which is equivalent to maximizing the goal-conditioned reward $r_g(x, y)$, i.e.,
\#\label{eq_obj}
\min_\pi\EE_{g, x\sim\mathcal{D}_N, y\sim\pi(\cdot\mid x ; g)}\bigl[|r(x, y) - g|\bigr] = \max_\pi\EE_{g, x\sim\mathcal{D}, y\sim\pi(\cdot\mid x ; g)}\bigl[r_g(x, y)\bigr].
\#

To optimize the RHS of Equation \eqref{eq_obj}, we first observe that $r_g(x, y)=1$ only when the goal reward equals the actual reward $r(x, y)$ of the prompt $x$ and response $y$. Therefore, for each preference pair ${x^i, y_w^i, r_w^i, y_l^i, r_l^i}$ in $\mathcal{D}_N$, the non-zero goal $r_g$

construct preference pairs under the goals of . 

\begin{figure*}[htbp]
    \centering
    \includegraphics[width=\linewidth]{figs/illu.pdf}
  \caption{Construction of the reward-augmented preference data.}
    \label{fig_illu}
\end{figure*}

As illustrated in Figure \ref{fig_illu}, for each preference pair with index $i$ in $\mathcal{D}_N$, we can set two goals that correspond to the reward values of the chosen response $y_w^i$ and the rejected response $y_l^i$. Specifically, under the first goal of $g=y_w^i$, the relabeled rewards are $r_g(x, y_w^i)=1$ and $r_g(x, y_l^i)=0$. The chosen and rejected responses are thus the same, except that the preference is ranked by conditioning on $g=y_w^i$. Similarly, under the second goal of $g=y_l^i$, the relabeled rewards are $r_g(x, y_l^i)=1$ and $r_g(x, y_w^i)=0$. Thus, the chosen and rejected responses are now $y_w^i$ and $y_l^i$, respectively. By generating preference pairs conditioned on the goal reward of the chosen and rejected responses for each data, we obtain reward-augmented data of size $2N$. Finally, we can leverage any direct alignment algorithms, such as DPO \citep{rafailov2024direct}, on the new reward-augmented data.

In this work, we implement the reward-conditioned policy $\pi(y\mid x ; g)$ as the LLM with a system prompt (or a prefix before the user prompt $x$ if system prompts are not supported by the LLM) such as ``generate responses of score $g$". At inference time, the LLM is conditioned on the highest possible reward value, e.g., $g=10$, to generate the responses.

==> theory.tex <==
\section{Proof of Theorem \ref{thm:regret}}
\label{proof_thm}
\begin{algorithm}[H]
\caption{Self-Exploring Language Models (SELM; Theoretical Version)}
\begin{algorithmic}[1]\label{alg_se_theory}
\REQUIRE Reference model $\pi_{\text{ref}}$, preference dataset $\mathcal{D}_0 = \emptyset$, iterations $T$, optimism coefficient $\alpha$.
\FOR{iteration $t = 1, 2, \ldots, T$}
\STATE Sample $x_t \sim \nu$, $y_t^1 \sim \pi_t(\cdot \mid x)$, $y_t^2 \sim \pi_{\mathrm{ref}}(\cdot \mid x)$.
\STATE Update the preference data $\cD_t = \cD_{t-1} \cup \{(x_t, y_t^1, y_t^2)\}$
\STATE Train the LLM $\pi_{t + 1} = \argmax_{\pi} \{ -\mathcal{L}_{\text{DPO}}(\pi; \mathcal{D}_t) - \alpha \cdot \EE_{x\sim\nu} \EE_{y \sim \pi_{\mathrm{ref}}(\cdot \mid x)}[\log\pi(y \mid x)]\}$.
\ENDFOR 
\end{algorithmic}
\end{algorithm}


\begin{definition}[Preference-based GEC] \label{def:pgec}
    For the function class $\Pi$, we define the preference-based GEC (PGEC) as the smallest $d_{\mathrm{GPEC}}$ as
    \$
    & \sum_{t = 1}^T \EE_{(x, y, y') \sim (\nu, \pi_{\mathrm{ref}}, \pi_t)} \left[  \log \frac{\pi^*(y \given x)}{\pi_{\mathrm{ref}}(y \given x)} - \log \frac{\pi_t(y \given x)}{\pi_{\mathrm{ref}}(y \given x)} - \log \frac{\pi^*(y' \given x)}{\pi_{\mathrm{ref}}(y' \given x)} +  \log \frac{\pi_t(y' \mid x)}{\pi_{\mathrm{ref}}(y' \mid x)} \right] \notag \\
& \le \sqrt{d_{\mathrm{PGEC}} \sum_{t = 1}^T \sum_{\tau = 1}^{t - 1} \EE_{(x, y, y') \sim (\nu, \pi_{\mathrm{ref}}, \pi^\tau)} \left[  \log \frac{\pi^*(y \given x)}{\pi_{\mathrm{ref}}(y \given x)} - \log \frac{\pi^\tau(y \given x)}{\pi_{\mathrm{ref}}(y \given x)} - \log \frac{\pi^*(y' \given x)}{\pi_{\mathrm{ref}}(y' \given x)} +  \log \frac{\pi^\tau(y' \mid x)}{\pi_{\mathrm{ref}}(y' \mid x)} \right]^2 }  \\
& \qquad + 4\sqrt{ d_{\mathrm{PGEC}} T} .
    \$
\end{definition}

The definition of PGEC is a preference-based version of Generalized Eluder Coefficient (GEC) proposed by \citep{zhong2022gec}. Intuitively, both PGEC and GEC establish a crucial connection between \emph{prediction error} and \emph{in-sample estimation error}, effectively transforming regret minimization into an online estimation problem. For a comprehensive explanation and in-depth discussion, readers are directed to \citet{zhong2022gec}. A slight difference is that the PGEC here is defined with respect to the policy class, while the GEC in \citet{zhong2022gec} is defined with respect to the model or value class. These can be connected if we regard the implicit reward class $\log (\pi/\pi_{\mathrm{ref}})$ as the model or value class. As an important example, if we consider the log-linear function class $\Pi = \{\pi_\theta: \pi_\theta(y \mid x) \propto \exp( \langle \phi(x, y), \theta \rangle /\beta )\}$, we can show that $d_{\mathrm{PGEC}} = \tilde{O}(d)$ by the elliptical potential lemma \citep{abbasi2011improved,zhong2022gec}. Another remark is that here the PGEC is defined in the bandit formulation, and it can be naturally extended to the token-wise MDP formulation \citep{zhong2024dpo,rafailov2024r,xie2024exploratory} and further connects to the eluder dimension in the context of preference-based MDPs \citep{chen2022human,wang2023rlhf}.


\begin{proof}[Proof of Theorem \ref{thm:regret}]
We first decompose the regret as
\$
\mathcal{R}(T) & = \sum_{t = 1}^T [J(\pi^*) - J(\pi_t)] \\
& = \sum_{t = 1}^T \left( \EE_{x \sim \nu, y \sim \pi^*(\cdot \mid x)}\left[r(x, y) - \beta \log \frac{\pi^*(y \mid x)}{\pi_{\mathrm{ref}}(y \mid x)}\right] - \EE_{x \sim \nu, y \sim \pi_t(\cdot \mid x)}\left[r(x, y) - \beta \log \frac{\pi_t(y \mid x)}{\pi_{\mathrm{ref}}(y \mid x)}\right] \right)\\
& = \sum_{t = 1}^T \left( \EE_{x \sim \nu, y \sim \pi_{\mathrm{ref}}(\cdot \mid x)}\left[r(x, y) - \beta \log \frac{\pi^*(y \mid x)}{\pi_{\mathrm{ref}}(y \mid x)}\right] - \EE_{x \sim \nu, y \sim \pi_t(\cdot \mid x)}\left[r(x, y) - \beta \log \frac{\pi_t(y \mid x)}{\pi_{\mathrm{ref}}(y \mid x)}\right] \right),
\$
where the last line uses the fact that 
\# \label{eq:closed:form}
r(x, y) - \beta \log \frac{\pi^*(y \mid x)}{\pi_{\mathrm{ref}}(y \mid x)} = \beta \cdot \log Z_r(x), 
\#
which is independent of the response $y$. Rearranging the above regret decomposition, we have
\# \label{eq:220}
\mathcal{R}(T) & = \sum_{t = 1}^T \left( \EE_{x \sim \nu, y \sim \pi_{\mathrm{ref}}(\cdot \mid x)}\left[r(x, y) - \beta \log \frac{\pi^*(y \mid x)}{\pi_{\mathrm{ref}}(y \mid x)}\right] - \EE_{x \sim \nu, y \sim \pi_t(\cdot \mid x)}\left[r(x, y) - \beta \log \frac{\pi_t(y \mid x)}{\pi_{\mathrm{ref}}(y \mid x)}\right] \right) \notag \\
& = \sum_{t = 1}^T \EE_{x \sim \nu, y \sim \pi_{\mathrm{ref}}(\cdot \mid x)} \left[ \beta \log \frac{\pi_t(y \mid x)}{\pi^*(y \mid x)} \right]    \notag \\
& \qquad + \sum_{t = 1}^T \EE_{x \sim \nu, y \sim \pi_{\mathrm{ref}}(\cdot \mid x), y' \sim \pi_t(\cdot \mid x)} \left[ r(x, y) - \beta \log \frac{\pi_t(y \given x)}{\pi_{\mathrm{ref}}(y \given x)} - r(x, y') + \beta \log \frac{\pi_t(y' \mid x)}{\pi_{\mathrm{ref}}(y' \mid x)} \right] \notag \\
& = \sum_{t = 1}^T \EE_{x \sim \nu, y \sim \pi_{\mathrm{ref}}(\cdot \mid x)} \left[ \beta \log \frac{\pi_t(y \mid x)}{\pi^*(y \mid x)} \right]    \notag \\
& \qquad + \beta \sum_{t = 1}^T \EE_{(x, y, y') \sim (\nu, \pi_{\mathrm{ref}}, \pi_t)} \left[  \log \frac{\pi^*(y \given x)}{\pi_{\mathrm{ref}}(y \given x)} - \log \frac{\pi_t(y \given x)}{\pi_{\mathrm{ref}}(y \given x)} - \log \frac{\pi^*(y' \given x)}{\pi_{\mathrm{ref}}(y' \given x)} +  \log \frac{\pi_t(y' \mid x)}{\pi_{\mathrm{ref}}(y' \mid x)} \right],  
\#
where the last line uses \eqref{eq:closed:form}.
By the definition of PGEC in Definition~\ref{def:pgec}, we have
{
\# \label{eq:221}
& \sum_{t = 1}^T \EE_{(x, y, y') \sim (\nu, \pi_{\mathrm{ref}}, \pi_t)} \left[  \log \frac{\pi^*(y \given x)}{\pi_{\mathrm{ref}}(y \given x)} - \log \frac{\pi_t(y \given x)}{\pi_{\mathrm{ref}}(y \given x)} - \log \frac{\pi^*(y' \given x)}{\pi_{\mathrm{ref}}(y' \given x)} +  \log \frac{\pi_t(y' \mid x)}{\pi_{\mathrm{ref}}(y' \mid x)} \right] \notag \\
& \le \sqrt{d_{\mathrm{PGEC}} \sum_{t = 1}^T \sum_{\tau = 1}^{t - 1} \EE_{(x, y, y') \sim (\nu, \pi_{\mathrm{ref}}, \pi^\tau)} \left[  \log \frac{\pi^*(y \given x)}{\pi_{\mathrm{ref}}(y \given x)} - \log \frac{\pi^\tau(y \given x)}{\pi_{\mathrm{ref}}(y \given x)} - \log \frac{\pi^*(y' \given x)}{\pi_{\mathrm{ref}}(y' \given x)} +  \log \frac{\pi^\tau(y' \mid x)}{\pi_{\mathrm{ref}}(y' \mid x)} \right]^2 } \notag \\ 
& \qquad + 4 \sqrt{d_{\mathrm{PGEC}} T} \notag \\
& \le \frac{d_{\mathrm{PGEC}}}{4\eta} + \eta \sum_{t = 1}^T \sum_{\tau = 1}^{t - 1} \EE_{(x, y, y') \sim (\nu, \pi_{\mathrm{ref}}, \pi^\tau)} \left[  \log \frac{\pi^*(y \given x)}{\pi_{\mathrm{ref}}(y \given x)} - \log \frac{\pi^\tau(y \given x)}{\pi_{\mathrm{ref}}(y \given x)} - \log \frac{\pi^*(y' \given x)}{\pi_{\mathrm{ref}}(y' \given x)} +  \log \frac{\pi^\tau(y' \mid x)}{\pi_{\mathrm{ref}}(y' \mid x)} \right]^2, \notag \\
& \qquad + 4 \sqrt{d_{\mathrm{PGEC}} T},
\#}
where the last inequality follows from the fact that $\sqrt{xy} \le x/(4\eta) + \eta y$ for any $x, y, \eta > 0$.

By the updating rule of $\pi_{t + 1} = \argmax_{\pi} \{ -\mathcal{L}_{\text{DPO}}(\pi; \mathcal{D}_t) - \alpha \cdot \EE_{x\sim\nu} \EE_{y \sim \pi_{\mathrm{ref}}(\cdot \mid x)}[\log\pi(y \mid x)]\}$, we have
\$
 -\mathcal{L}_{\text{DPO}}(\pi_{t}; \mathcal{D}_{t-1}) - \alpha \cdot \EE_{x\sim\nu, y \sim \pi_{\mathrm{ref}}(\cdot \mid x)} [\log\pi_{t}(y \mid x)] \ge  -\mathcal{L}_{\text{DPO}}(\pi^*; \mathcal{D}_{t-1}) - \alpha \cdot \EE_{x\sim\nu, y \sim \pi_{\mathrm{ref}}(\cdot \mid x)}[\log\pi^*(y \mid x)],
\$
which equivalents to that
\# \label{eq:222}
\EE_{x\sim\nu, y \sim \pi_{\mathrm{ref}}(\cdot \mid x)} \left[ \beta \log \frac{\pi_t(y \mid x)}{\pi^*(y \mid x)} \right] \le \frac{\beta}{\alpha} \cdot \left( \cL_{\mathrm{DPO}}(\pi^*; \cD_{t-1}) - \cL_{\mathrm{DPO}}(\pi_t; \cD_{t-1}) \right). 
\#
We upper bound the right handsise of \eqref{eq:222} via the following lemma.
\begin{lemma}[Concentration] \label{lemma:concentration}
For any $t \in [T]$ and $0 < \delta < 1$, it holds with probability $1- \delta$ that
\$
& \cL_{\mathrm{DPO}}(\pi^*; \cD_{t-1}) - \cL_{\mathrm{DPO}}(\pi_t; \cD_{t-1}) \\
& \lesssim -\frac{2}{\exp(4R_{\max})} \cdot \sum_{\tau = 1}^{t - 1} \EE_{(x, y, y') \sim (\nu, \pi_{\mathrm{ref}}, \pi^\tau)} \left[  \log \frac{\pi^*(y \given x)}{\pi_{\mathrm{ref}}(y \given x)} - \log \frac{\pi^\tau(y \given x)}{\pi_{\mathrm{ref}}(y \given x)} - \log \frac{\pi^*(y' \given x)}{\pi_{\mathrm{ref}}(y' \given x)} +  \log \frac{\pi^\tau(y' \mid x)}{\pi_{\mathrm{ref}}(y' \mid x)} \right]^2 \\
&  \qquad + \log(|\Pi|/\delta).
\$
\end{lemma}

\begin{proof}
    The proof of this lemma follows the standard MLE analysis \citep{zhang2006varepsilon} and its application for standard reward-based RL \citep{agarwal2020flambe,liu2024maximize}. Recent works \citep{liu2024provably,xie2024exploratory,cen2024value} also applies this result for RLHF. For brevity, we omit the detailed proof here and direct readers to these related works for the proof.
\end{proof}

Combining \eqref{eq:220}, \eqref{eq:221}, \eqref{eq:222}, and Lemma~\ref{lemma:concentration}, together with the parameter choice $\alpha = 2/(\eta \exp(4R_{\max}))$, we obtain
\$
\cR(T) &\lesssim \frac{\beta T d_{\mathrm{PGEC}}}{\eta} + \beta \eta \cdot {\exp(4R_{\max})} \log (|\Pi|/\delta) + 4 \sqrt{d_{\mathrm{PGEC}} T} \\
& \lesssim \sqrt{d_{\mathrm{PGEC}} \cdot \exp(2R_{\max}) \cdot T \cdot \log (|\Pi|/\delta)},
\$
where the last line follows from the fact that $\eta = \sqrt{T d_{\mathrm{PGEC}}/(\exp(4R_{\max}) \log(|\Pi|/\delta)) }$. Therefore, we finish the proof of Theorem~\ref{thm:regret}.
\end{proof}
